Optimizing Dense Retrieval Model Training with Hard Negatives

Ranking has always been one of the top concerns in information retrieval researches. For decades, the lexical matching signal has dominated the ad-hoc retrieval process, but solely using this signal in retrieval may cause the vocabulary mismatch problem. In recent years, with the development of representation learning techniques, many researchers turn to Dense Retrieval (DR) models for better ranking performance. Although several existing DR models have already obtained promising results, their performance improvement heavily relies on the sampling of training examples. Many effective sampling strategies are not efficient enough for practical usage, and for most of them, there still lacks theoretical analysis in how and why performance improvement happens. To shed light on these research questions, we theoretically investigate different training strategies for DR models and try to explain why hard negative sampling performs better than random sampling. Through the analysis, we also find that there are many potential risks in static hard negative sampling, which is employed by many existing training methods. Therefore, we propose two training strategies named a Stable Training Algorithm for dense Retrieval (STAR) and a query-side training Algorithm for Directly Optimizing Ranking pErformance (ADORE), respectively. STAR improves the stability of DR training process by introducing random negatives. ADORE replaces the widely-adopted static hard negative sampling method with a dynamic one to directly optimize the ranking performance. Experimental results on two publicly available retrieval benchmark datasets show that either strategy gains significant improvements over existing competitive baselines and a combination of them leads to the best performance.

==> theory/notion_table.tex <==
\begin{table}[t]
    \centering
    \caption{The commonly used notions.}
    \label{tab:notions}
    \begin{tabular}{ll} \hlinew{0.8pt}
    \textbf{Notions} & \textbf{Descriptions} 
    \\ \hline
    
    $q$             & A query. \\
    $C$   			& Corpus. \\
    $d$             & A document.  \\
    $d_q$           & The relevant document of query $q$. \\
    $\mathcal{A}(q,d)$       & The relevance label of $q$ and $d$. \\
    $\theta$        & The parameter weights of the DR model. \\
    $\vv{X}_{q;\theta}$ & The output embedding of $q$. \\
    $\vv{X}_{d;\theta}$ & The output embedding of $d$. \\
    ${\rm s}(q, d ; \theta)$ & The predicted relevance score of $q$ and $d$. \\
    ${\rm R_q}(d ; \theta)$  & $d$'s position in $q$'s ranking list. \\
    $\mathcal{L}(q,d,d_q ; \theta)$ & The pairwise loss. \\
    $\mathcal{D}_{q;\theta}$ & The negative documents for query $q$. \\
    $w(q,d ; \theta)$        & The normalized weight for $d \in \mathcal{D}_{q;\theta}$ \\
    $\mathcal{N}$            & A negative sampling training method. \\
    $\theta | \mathcal{N}$   & The optimal parameter weights for $\mathcal{N}$. \\
    $\mathcal{M}(q;\theta)$  & The evaluation score for query $q$. \\
    $f_\mathcal{M}$          & $\mathcal{M}(q;\theta) = f_\mathcal{M}({\rm R_q}(d_q ; \theta))$ \\
\hlinew{0.8pt} 
    \end{tabular}
\end{table}




